Novel Approach to Measure Motion-To-Photon and Mouth-To-Ear Latency in Distributed Virtual Reality Systems

Distributed Virtual Reality systems enable globally dispersed users to interact with each other in a shared virtual environment. In such systems, different types of latencies occur. For a good VR experience, they need to be controlled. The time delay between the user's head motion and the corresponding display output of the VR system might lead to adverse effects such as a reduced sense of presence or motion sickness. Additionally, high network latency among worldwide locations makes collaboration between users more difficult and leads to misunderstandings. To evaluate the performance and optimize dispersed VR solutions it is therefore important to measure those delays. In this work, a novel, easy to set up, and inexpensive method to measure local and remote system latency will be described. The measuring setup consists of a microcontroller, a microphone, a piezo buzzer, a photosensor, and a potentiometer. With these components, it is possible to measure motion-to-photon and mouth-to-ear latency of various VR systems. By using GPS-receivers for timecode-synchronization it is also possible to obtain the end-to-end delays between different worldwide locations. The described system was used to measure local and remote latencies of two HMD based distributed VR systems.

==> Chapter/MethodDescription_BACKUP.tex <==
\section{Method Description}
In the following section the measuring system will be explained in detail. 

\subsection{Rotation platform}
For the measurement setup, a potentiometer is used to continuously trace the rotation angle of the tracked object (e.g. an HMD). The platform rotary motion is controlled by a servo connected to the microcontroller. With this setup, steady back-and-forth movements of the tracked object are possible.

\subsection{Photosensor}
\label{sec:photosensor}
The photosensor is used to monitor display outputs and capture the rotary angle of the tracking system which is output in a brightness code.

During measurement, right before the rendering process, the VR system outputs the last captured horizontal rotation angle in a encoded brightness code. To get a resolution of 4096  different values, four areas on the display are used to output a number in the octal numeral system. By capturing each area with a light sensitive sensor connected to the microcontroller, it is possible to get the rotation angle output of the VR system at every interval.

The base-8 numeral system is used because the analogue signal of the photosensors is noisy and a bit of headroom between the different brightness levels is needed. 

The whole photosensor consists of four \textit{TSL250R} photosensors which are very similar to those used in \textit{Di Luca's Method}~\cite{DiLuca.2010}. According to the datasheet the sensors have an output rise-time of about 260 $\mu s$~\cite{TAOSInc..2001}. 

With the HMDs, like the \textit{Oculus CV1} used in this work, it is not possible to directly attach the photosensor to the VR display without the need to disassemble the hardware. HMDs use optical lenses in front of the display system to expand the field of view. Without any light path correction it is not possible to get a sharp image of the displayed frame on a flat surface like the one of the photosensor.

To read the brightness code of the VR system on HMDs, an additional optical lens is necessary. For the measurement setup, convex lenses built into the low-cost VR glasses \textit{Google Cardboard} where directly attached to the lenses of the HMD to correct the light path of the VR display. Attaching the photosensor a few millimetre away from the correction lens makes it possible to get read the displayed brightness code. 

%TODO bild
%TODO display types

\subsection{Audio Latency Detector}
To detect the mouth-to-ear latency of VR systems, a combination of piezo buzzer and microphone is used. 

By attaching the buzzer to an analogue output pin with pulse-width modulation (PWM) capability of the microcontroller, a square wave signal was generated to get a simple tone. For the described setup an audio frequency of 4~kHz was used since at this frequency the sound pressure output of the used piezo buzzer was at it's maximum. The buzzer is attached to the microphone of the VR simulation.

In order to detect the generated tone at the speakers of the VR system, a cheap sound detection model is used. The \textit{SparkFun Sound Detector}\footnote{\url{https://github.com/sparkfun/Sound_Detector}} consists of a simple electret microphone, a voltage feedback amplifier, and a comparator. If the sound pressure at the detection module reaches a specific threshold which can be adjusted with a built-in potentiometer, the digital output pin of the module is set to high. One digital pin of the microcontroller is used as input pin and waits for a rising signal of the sound detection module. When a high signal is detected, the elapsed intervals since activating the buzzer are summed up and represent the measured mouth-to-ear delay.

\subsection{Microcontroller} 
As central unit of the external measuring system, \textit{Teensy~3.2} microcontrollers\footnote{\url{https://www.pjrc.com/store/teensy32.html}} are used. With the built-in 16~Mhz crystal~\cite{PJRC.} continuous measurements with a stable frequency are possible. Since the crystal clock accuracy is unspecified, a worst-case quality for quartz crystals of $\pm$100~ppm is assumed, even though the actual accuracy is expected to be significantly better than this ($\pm$15~ppm\footnote{\url{"https://forums.adafruit.com/viewtopic.php?f=24&t=84843"}}). With the assumed worst-case accuracy, it is possible to measure with a maximum time deviation of $\pm$0.5~ms over a timespan of 5~s.
%TODO \textit{Teensy 3.2} internal accuracy 15ppm %https://forums.adafruit.com/viewtopic.php?f=24&t=84843
%TODO Arduino Uno Ceramic Resonator https://rheingoldheavy.com/arduino-from-scratch-part-10-atmega328p-subsystem/

The photosensors and the potentiometer are connected to the analogue inputs of the microcontroller. The built-in analogue-to-digital converter (ADC) of the \textit{Teensy~3.2} is used to capture all sensor inputs and store them in the microcontroller's Random Access Memory (RAM). All analogue-to-digital conversions of the connected sensors take less than 1~ms. Therefore, continuous measurements can be done with a frequency of 1000~Hz. 

A frequency of 1~kHz is used, because of the built-in OLED displays of current HMDs. Those displays show a new frame only between 1~ms and 2~ms until the display turns black again.

Theoretically, even higher measure frequencies are possible, but for the described VR scenarios 1~ms intervals proved to be fast enough. Capturing with higher frequencies would also require extra RAM space.

\subsection{Synchronization}
To measure the delay between different worldwide locations, synchronized timecodes are needed. Unlike with the method described by \textit{Roberts et al.}~\cite{Roberts.b}, synchronizing both devices at the same location before measurement is not necessary because GPS-receivers are used. 

For the described setup two \textit{u-blox NEO-6M} modules continuously transmit GPS data to the connected microcontrollers. This data contain an \textit{UTC timestamp} which is used for synchronization. Beside the serial connection for the GPS data, the \textit{u-blox NEO-6M} has another pin which outputs a very accurate timepulse signal that rises every full second with an root-mean-square accuracy of 30~$\mu s$~\cite{UBloxAG.2011}. Figure \ref{fig:Timepulse} shows how the signal is used to get highly-accurate GPS timestamps. 

\begin{figure} [h!]
	\centering
	\begin{tikzpicture}[
	arrow/.style={<->,>=stealth',shorten >=1pt,semithick},
	arrowOneEnd/.style={->,>=stealth',shorten >=1pt,semithick},
	line/.style={line width = 0.2mm},
	pulse/.style={line width = 0.6mm}
	]
	
	\draw[line] (0,1)-- (1,1);
	\draw[pulse] (1,1)-- (1,2);
	\draw[line] (1,2)-- (2,2);
	\draw[line] (2,2)-- (2,1);
	\draw[line] (2,1)-- (5,1);
	\draw[pulse] (5,1)-- (5,2);
	\draw[line] (5,2)-- (6,2);
	\draw[line] (6,2)-- (6,1);
	\draw[line] (6,1)-- (7,1);
		
	% One Second
	\draw [arrow] (1,0) -- (5,0);
	\node [align=center, below](1s) at (3,0) {\small 1000 ms};
	
	% Time Pulse
	\draw [arrow] (1,0.7) -- (2,0.7);
	\node [align=center, below](1s) at (1.5,0.7) {\small 100 ms};
	\draw [arrow] (5,0.7) -- (6,0.7);
	\node [align=center, below](1s) at (5.5,0.7) {\small 100 ms};
	
	% Time GPS	
	\draw [arrowOneEnd] (1,2.3) -- (1,2);
	\node [align=center, above](1s) at (1,2.3) {\small GPS 10:20:00};
	\draw [arrowOneEnd] (5,2.3) -- (5,2);
	\node [align=center, above](1s) at (5,2.3) {\small GPS 10:20:01};
		
	\end{tikzpicture}
	\caption {Timepulse signal for GPS time synchronization}
	\label{fig:Timepulse} 
\end{figure}

If two or more microcontrollers are synchronized to GPS time, an UTC timestamp can be transmitted to the controllers. All globally-distributed systems will wait until that time and then start taking measurements simultaneously. 

%TODO GPS Test
%GPS-Timestamp + RTC (Auch ohne GPS)
%TODO Internal crystal ~100 ppm? -> 0.1 ms / s
%- Accuracy $\pm$2ppm from 0$^{\circ}$C to +40$^{\circ}$C \\
%- Accuracy $\pm$3.5ppm from -40$^{\circ}$C to +85$^{\circ}$C~\cite{MaximIntegratedProducts.2015}
%RTC 2ppm = +-7,2 ms / h

%inconsistency occurs at site 0 due to the deviating clocks. Typical values for time deviation of computers using NTP or SNTP are 20-50 ms if the NTP server is reached via WAN and less than 10 ms if the NTP server is part of the same LAN.

\subsection{Data evaluation}
After measurement, the raw data captured with the microcontrollers are transmitted to the VR simulation computer. Using \textit{Unity 3D} scripts, the photosensor data of all four photosensors are decoded into the corresponding decimal number which represents the rotation output of the VR system.

Then three files are generated. Two files contain the display output and the rotation platform data. The last file contains the measured audio latency.

\texttt{R} scripts are used to calculate motion-to-photon latency. The recorded potentiometer and photosensor data are cross-correlated with each other. Since the described system captures data with a frequency of 1000~Hz one interval has the length of 1~ms. Therefore, determining the interval for the maximum correlation coefficient is used as measured motion-to-photon latency.

\begin{figure} [h!]
	\centering
	\includegraphics[width=\columnwidth]{Latency_OCR}
	\caption {Motion-to-photon latency Oculus Rift CV 1}
	\label{fig:DataEvaluation} 
\end{figure}

Figure \ref{fig:DataEvaluation} shows an example of the measured motion-to-photon latency of the \textit{Oculus Rift CV1}. The blue line represents the captured rotation of the potentiometer and the red line is the corresponding display output. For the example in figure \ref{fig:DataEvaluation} the maximum correlation, and therefore the estimated motion-to-photon latency, was at 8~ms.
